Grappa -- A Machine Learned Molecular Mechanics Force Field

Simulating large molecular systems over long timescales requires force fields that are both accurate and efficient. In recent years, E(3) equivariant neural networks have lifted the tension between computational efficiency and accuracy of force fields, but they are still several orders of magnitude more expensive than established molecular mechanics (MM) force fields. Here, we propose Grappa, a machine learning framework to predict MM parameters from the molecular graph, employing a graph attentional neural network and a transformer with symmetry-preserving positional encoding. The resulting Grappa force field outperformstabulated and machine-learned MM force fields in terms of accuracy at the same computational efficiency and can be used in existing Molecular Dynamics (MD) engines like GROMACS and OpenMM. It predicts energies and forces of small molecules, peptides, RNA and - showcasing its extensibility to uncharted regions of chemical space - radicals at state-of-the-art MM accuracy. We demonstrate Grappa's transferability to macromolecules in MD simulations from a small fast folding protein up to a whole virus particle. Our force field sets the stage for biomolecular simulations closer to chemical accuracy, but with the same computational cost as established protein force fields.

==> content/tables/amber_compatibility.tex <==
\begin{tabular}{ccc|cc}
    \hline
    \hline
    \multicolumn{3}{c|}{{Learnable contribution}} & \multicolumn{2}{c}{{RMSE [kcal/mol(/Å)]}} \\
    \hline
    Bond & Angle & Dihedral & Energy & Force \\
    \hline
\checkmark & \checkmark & \checkmark & 2.4 & 5.8 \\ 
\checkmark & \checkmark &  & 3.1 & 6.5 \\ 
\checkmark &  &  & 3.6 & 8.8 \\ 
 & \checkmark &  & 3.5 & 11.2 \\ 
 &  & \checkmark & 3.8 & 12.2 \\ 
 &  &  & 4.1 & 11.8 \\ 

    \hline
    \hline
\end{tabular}

==> content/tables/full_benchmark.tex <==

% Define variables for vertical spacing
\newcommand{\widthbetweentype}{7pt}


\begin{tabular*}{\textwidth}{l c c l c c c c c c}

        \hline
        \hline
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Test Mols} & \multirow{2}{*}{Confs} & & \multirow{2}{*}{Grappa} & \multirow{2}{*}{Espaloma} & \multirow{2}{*}{Gaff-2.11} & ff14SB, & Mean\\
        & & & & & & & RNA.OL3 & Predictor\\
        \hline
        \multicolumn{8}{l}{\vspace{\widthbetweentype}} \\[-1em]
        \multicolumn{8}{l}{\small{BOLTZMANN SAMPLED}} \\\hline
        \multirow{2}{*}{SPICE-Pubchem} & \multirow{2}{*}{1411} & \multirow{2}{*}{60853} & \textit{Energy} & \textbf{2.3} & \textbf{2.3} & 4.6 &  & 18.4\\
                                           &                       &                         & \textit{Force}  & \textbf{6.1} & 6.8 & 14.6 &  & 23.4\\
        \hline
        \multirow{2}{*}{SPICE-DES-Monomers} & \multirow{2}{*}{39} & \multirow{2}{*}{2032} & \textit{Energy} & \textbf{1.3} & 1.4 & 2.5 &  & 8.2\\
                                           &                       &                         & \textit{Force}  & \textbf{5.2} & 5.9 & 11.1 &  & 21.3\\
        \hline
        \multirow{2}{*}{SPICE-Dipeptide} & \multirow{2}{*}{67} & \multirow{2}{*}{2592} & \textit{Energy} & \textbf{2.3} & 3.1 & 4.5 & 4.6 & 18.7\\
                                           &                       &                         & \textit{Force}  & \textbf{5.4} & 7.8 & 12.9 & 12.1 & 21.6\\
        \hline
        \multirow{2}{*}{RNA-Diverse} & \multirow{2}{*}{6} & \multirow{2}{*}{357} & \textit{Energy} & \textbf{3.3} & 4.2 & 6.5 & 6.0 & 5.4\\
                                           &                       &                         & \textit{Force}  & \textbf{3.7} & 4.4 & 16.7 & 19.4 & 17.1\\
        \hline
        \multirow{2}{*}{RNA-Trinucleotide} & \multirow{2}{*}{64} & \multirow{2}{*}{35811} & \textit{Energy} & \textbf{3.5} & 3.8 & 5.9 & 6.1 & 5.3\\
                                           &                       &                         & \textit{Force}  & \textbf{3.6} & 4.3 & 17.1 & 19.7 & 17.7\\
        \hline
        \multicolumn{8}{l}{\vspace{\widthbetweentype}} \\[-1em]
        \multicolumn{8}{l}{\small{TORSION SCAN}} \\\hline
        \multirow{2}{*}{Gen2-Torsion} & \multirow{2}{*}{131} & \multirow{2}{*}{21890} & \textit{Energy} & 1.7 & \textbf{1.6} & 2.7 &  & 4.7\\
                                           &                       &                         & \textit{Force}  & \textbf{4.0} & 4.7 & 9.4 &  & 5.5\\
        \hline
        \multirow{2}{*}{Protein-Torsion} & \multirow{2}{*}{9} & \multirow{2}{*}{6624} & \textit{Energy} & 2.2 & \textbf{1.9} & 3.0 &  & 3.5\\
                                           &                       &                         & \textit{Force}  & 3.8 & \textbf{3.5} & 9.7 &  & 5.1\\
        \hline
        \multicolumn{8}{l}{\vspace{\widthbetweentype}} \\[-1em]
        \multicolumn{8}{l}{\small{OPTIMIZATION}} \\\hline
        \multirow{2}{*}{Gen2-Opt} & \multirow{2}{*}{154} & \multirow{2}{*}{40055} & \textit{Energy} & 1.8 & \textbf{1.7} & 3.0 &  & 3.9\\
                                           &                       &                         & \textit{Force}  & \textbf{3.8} & 4.5 & 9.7 &  & 5.1\\
        \hline
        \multirow{2}{*}{Pepconf-Opt} & \multirow{2}{*}{55} & \multirow{2}{*}{14884} & \textit{Energy} & 3.2 & \textbf{2.8} & 5.1 & 4.1 & 6.3\\
                                           &                       &                         & \textit{Force}  & \textbf{3.6} & 4.0 & 10.2 & 10.2 & 5.3\\
        \hline
        \hline
        \hline
\end{tabular*}


==> icml_style/header_icmlstyle_old.tex <==
% CHANGES CAN BE FOUND BY SEARCHING FOR "NOTE"
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure} % NOTE: conflict with subcaption
\usepackage{booktabs} % for professional tables

% \usepackage{natbib} % NOTE: we change these to numerical references
\usepackage[numbers, compress]{natbib} % Use numerical citations

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2024} with \usepackage[nohyperref]{icml2024} above.
\usepackage{hyperref}


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
\usepackage{icml_style/icml2024}

% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{icml_style/icml2024}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
% \usepackage[textsize=tiny]{todonotes}


% The \icmltitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
\icmltitlerunning{\input{content/title.tex}}
\usepackage{times}
